Expert-elicitation method for non-parametric joint priors using normalizing flows

We propose an expert-elicitation method for learning non-parametric joint prior distributions using normalizing flows. Normalizing flows are a class of generative models that enable exact, single-step density evaluation and can capture complex density functions through specialized deep neural networks. Building on our previously introduced simulation-based framework, we adapt and extend the methodology to accommodate non-parametric joint priors. Our framework thus supports the development of elicitation methods for learning both parametric and non-parametric priors, as well as independent or joint priors for model parameters. To evaluate the performance of the proposed method, we perform four simulation studies and present an evaluation pipeline that incorporates diagnostics and additional evaluation tools to support decision-making at each stage of the elicitation process.

==> tables/table_1.tex <==
\begin{table}[h!]
\begin{tabular}{p{0.4\textwidth} p{0.5\textwidth}}
\hline
\emph{Symbol}  &  \emph{Description}\\
\hline
\multicolumn{2}{l}{Simulation-based prior elicitation}\\
\hline
$y_n$ & data $n = 1, \ldots, N$\\
$\theta_k$ & model parameter $k=1,\ldots,K$ \\
$\lambda$ & model hyperparameter \\
$p(y \mid \theta)$  & likelihood \\
$p(\theta \mid \lambda)$ & prior parameterized by $\lambda$ \\
$p(y)$ & prior predictive distribution \\
$z_i = c_i(\lambda)$ & simulated model target quantity defined by function $c_i$ \\
$\hat z_i$ & expert representation of the target quantity \\
$t_m = f_j(z_i)$ & model-elicited statistic defined by elicitation technique $f_j$\\
$\hat t_m$ & expert-elicited statistic \\
$L_m(t_m(\lambda),\hat t_m)$ & loss component \\
$L(\lambda)=\sum_{m=1}^M\alpha_m L_m(t_m(\lambda),\hat t_m)$ & total loss as weighted sum of $L_m$ with weights $\alpha_m$\\
$p_{\lambda_1,\ldots,\lambda_R}(\theta)=\sum_{r=1}^R w_r \cdot p_{\lambda_r}(\theta)$ & averaged prior across $R$ replications and weighted by $w_r$ with $r=1,\ldots,R$\\
$\Delta_r(L) = L(\lambda_r)-L(\lambda_{\min})$ & difference between total loss of replication $r$ and replication with minimum total loss \\
$w_r = \frac{\exp\{-\gamma \Delta_r(L)\}}{\sum_{v=1}^V\exp\{-\gamma \Delta_v(L)\}}$ & weights used for model averaging with $\gamma$ being a scaling factor; in all simulation studies $\gamma=1.$\\
\hline
\multicolumn{2}{l}{Normalizing flow} \\
\hline
$u\sim p_U(u)$ & samples from base distribution \\
$g_\lambda(\cdot)$ & generator function \\
$u = g_\lambda(\theta)$ & normalizing direction \\
$\theta = g^{-1}_\lambda(u)$ & generative direction \\
$g_\lambda = g_{\lambda_H} \circ \cdots \circ g_{\lambda_1}$ & composition of $H$ coupling layers\\
\hline
\end{tabular}
\caption{Notation and symbols used in this paper.}
\label{tab:symbols}
\end{table}

==> tables/table_2.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{p{0.24\textwidth} p{0.24\textwidth} p{0.43\textwidth}}
    \hline 
    \\[-0.8em]
    \emph{Model}  & \emph{Generative Model} & \emph{Ground Truth} \\[0.4em]
    \hline
    \\[-0.8em]
    Binomial --- M1 & $y_i \sim \text{Binomial}(p_i, 30)$ & $\beta_0 \sim \text{Normal}(0.1, 0.1)$ \\
    (Section~\ref{subsec:binomial}) & $p_i = \text{sigmoid}(\beta_0+\beta_1x_i)$ & $\beta_1 \sim \text{Normal}(-0.1, 0.3)$ \\[0.4em]
    \hline
    \\[-0.8em]
    \textbf{Normal models} &  & \\
    \quad \emph{Scenario 1} --- M2 & $y_i \sim \text{Normal}(\mu_i, \sigma)$ & $\beta_0 \sim~\text{Normal}(10, 2.5)$ \\
     \quad (Section~\ref{subsec:independent-normal}) & $\mu_i = \beta_0+\beta_1 x_{1,i}+\beta_2 x_{2,i}$ & $\beta_1 \sim \text{Normal}(7, 1.3)$\\
     && $\beta_2 \sim \text{Normal}(2.5, 0.8)$ \\
     && $\sigma \sim \text{Gamma}(5, 2)$ \\[0.4em]
     \hdashline
     \\[-0.8em]
     \quad \emph{Scenario 2} --- M3 & see M2 & $\beta_0 \sim~\text{Normal}(10, 2.5)$\\
     \quad (Section~\ref{subsec:skewed-normal}) && $\beta_1 \sim \text{SkewNormal}(7, 1.3, 4)$\\
     && $\beta_2 \sim \text{SkewNormal}(2.5, 0.8, 4)$ \\
     && $\sigma \sim \text{Gamma}(5, 2)$ \\[0.4em]
     \hdashline 
     \\[-0.8em]
     \quad \emph{Scenario 3} --- M4 \\[-1.3em] \quad (Section~\ref{subsec:correlated-normal})& see M2 & $\beta \sim \text{Mv-Normal}\left(\begin{bmatrix}  10 \\ 7 \\ 2.5\end{bmatrix}, \; \text{D}(s) \, \textbf{R} \, \text{D}(s)\right)$ \\
      && $\textbf{R} = \begin{bmatrix} 1. & 0.3 & -0.3 \\
            0.3 & 1. & -0.2 \\ -0.3 & -0.2 & 1. \end{bmatrix}$\\
    && $s = ( 2.5 , 1.3 , 0.8 )$\\
    && $\sigma \sim \text{Gamma}(5, 2)$ \\
    \hline
    \end{tabular}
    \caption{Overview of generative models and ground truth in the simulation studies. Symbols: $\mathbf{R}$ denotes the correlation matrix and $s$ the vector of standard deviations.}
    \label{tab:overview-models}
\end{table}

==> tables/table_3.tex <==
\begin{table}[h!]   
    \begin{tabular}{p{0.24\textwidth} p{0.24\textwidth} p{0.43\textwidth}}
        \hline \\[-0.5em]
         \emph{Task} & \emph{Approach} & \emph{Insights} \\[0.3em]
         \hline
         \multicolumn{3}{l}{\textbf{Setup \& Elicitation Stage}}\\
         \hline
         Select the set of elicited statistics and evaluate its informativeness. & (1) Simulate elicited statistics by defining a true joint prior (i.e., the oracle). (2) Conduct a sensitivity analysis. & Can the set of elicited statistics provide sufficient information to learn the key aspects of the joint prior? \\
         \hline
         \multicolumn{3}{l}{\textbf{Fitting Stage}}\\
         \hline
         Evaluate variability in learned priors to assess non-identifiability. & Run the training algorithm several times with different random seeds. & Do different training runs yield different results?\\
         \hdashline
         Verify convergence of the training algorithm. & (1) Examine the slope of final loss values across replications. (2) Visually check the convergence of key quantities for selected seeds. & Will training the model for additional epochs lead to a practically relevant improvement in performance or a reduction in total loss? \\
         \hdashline
         Verify accurate learning of expert data. & Visually compare model-implied and expert-elicited statistics. & Was the method successful in accurately capturing the expert data? \\
         \hline
         \multicolumn{3}{l}{\textbf{Evaluation Stage}}\\
         \hline
         Examine the learned priors across the different seeds & Visually inspect the marginal priors and correlations between model parameters. & How much do the learned priors vary between different seeds? Were any degenerate prior distributions learned? Do we observe any form of multi-modality? Can any of the learned priors be ruled out as unreasonable post hoc? \\
         \hdashline
         Obtain the final learned prior for subsequent analysis. & Perform model averaging using weights based on relative loss performance. & Instead of selecting a single prior, compute a model average over practically equivalent priors to account for additional variability due to non-identifiability. \\
         \hline
    \end{tabular}
    \caption{Overview of the analysis workflow used in the simulation studies.}
    \label{tab:analysis_workflow}
\end{table}
